Quantum Tutte Embeddings

Using the framework of Tutte embeddings, we begin an exploration of \emph{quantum graph drawing}, which uses quantum computers to visualize graphs. The main contributions of this paper include formulating a model for quantum graph drawing, describing how to create a graph-drawing quantum circuit from a given graph, and showing how a Tutte embedding can be calculated as a quantum state in this circuit that can then be sampled to extract the embedding. To evaluate the complexity of our quantum Tutte embedding circuits, we compare them to theoretical bounds established in the classical computing setting derived from a well-known classical algorithm for solving the types of linear systems that arise from Tutte embeddings. We also present empirical results obtained from experimental quantum simulations.

==> np.tex <==
\section{Force-Direct Graph Drawing is NP-hard}

% Split solvable and general cases into definitions that can be referenced in later sections. 

Suppose we are given a graph, $G=(V,E)$.
In a common particle-and-spring framework for
force-directed graph drawing (e.g., 
see the classic paper by Fructerman 
and Reingold~\cite{fruchterman1991graph}
or the book by 
{Di Battista}, Eades, Tamassia, and Tollis~\cite{battista1999graph}),
$G$ is assigned a \emph{placement}, $\Gamma$, so that
each vertex, $v\in V$, is assigned to a point, $p_v$, in the plane, and each
edge $(u,v)\in E$ is assigned to a closed curve (which is typically a straight
line segment) joining $p_u$ and $p_v$.
For each edge, $(u,v)$ in $E$, there is an attractive (spring) force,
$F^{(a)}_{u,v}(p_u,p_v)$, and for every pair, $u,v\in V\times V$,
there is a repulsive (particle) force,
$F^{(r)}_{u,v}(p_u,p_v)$.
The goal of force-directed graph drawing is to
find a placement, $\Gamma$, for $G$ that minimizes the total energy,
\begin{equation}
\mathbb{E}_\Gamma 
= \sum_{(u,v)\in E} F^{(a)}_{u,v}(p_u,p_v) ~~+~
\sum_{(u,v)\in V\times V} F^{(r)}_{u,v}(p_u,p_v) .
\label{eq-forces}
\end{equation}

There are a number of algorithms for 
finding a placement, $\Gamma$, that minimizes $\mathbb{E}_{\Gamma}$,
e.g., see~\cite{bannister2013force,battista1999graph,fruchterman1991graph,gajer2004multi,hu2005efficient,kamada1989algorithm,kobourov2013}.
Most of these algorithms are not guaranteed to find such an optimal
placement, however, and instead use various heuristics to come close
to an optimal value.
For example, the only class of algorithms we are familiar
with that are guaranteed to find an optimal placement are 
based on a classic force-directed approach of 
Tutte~\cite{tutte1963draw},
e.g., as generalized by Hopcroft and Kahn~\cite{hopcroft1992paradigm} to
stressed graphs, 
% \begin{definition}\cite{tutte1963draw}\label{def:tutte}
% Let $G$ be a 3-connected planar graph, 
where we fix the vertices 
of an external face of a 3-connected planar graph, $G$, as a convex polygon,
and define $F^{(r)}_{u,v}(p_u,p_v)=0$ and 
$F^{(a)}_{u,v}(p_u,p_v)$ to be a simple spring 
force with positive weight, $w_{u,v}$, and idealized length $0$.
% \end{definition}

The lack of optimal methods in the general case is at least partly due
to the fact that,
as shown by Bannister, Devanny, Eppstein, and 
Goodrich~\cite{bannister2014galois},
Galois theory implies 
that many variants of force-directed graph drawing
have optimal solutions that cannot be expressed by nested 
radicals or nested roots of low-degree polynomials; 
hence, such optinmal solutions cannot be computed exactly 
even in extended computational models that include such operations.
In addition, we have the following, which may be part of the Graph
Drawing folklore, but we nevertheless include it for the sake of completeness.

\begin{theorem}
Optimal force-directed graph drawing is NP-hard.
\end{theorem}

\begin{proof}
Let us formally define 
the ``Optimal Force-Directed Graph Drawing'' problem as 
a decision problem where, in addition to a graph $G$ and 
force functions, $F^{(a)}$ and $F^{(r)}$,
we are given an energy value, $\mathbb{E}$, and we are asked if there exists
a placement $\Gamma$ such that,
for $\mathbb{E}_\Gamma$ defined as above in (\ref{eq-forces}),
$\mathbb{E}_\Gamma\le \mathbb{E}$.
Eades and Wormald~\cite{eades1990fixed} show that, given a
2-connected planar graph, $G$, it is NP-hard to determine whether 
there is a planar drawing of $G$ such that each edge has length 
exactly $1$.
(See also Cabello, Demaine, and Rote~\cite{sergio}.)
Suppose, therefore, for the sake of a reduction from this problem,
we are given a 2-connected planar graph, $G$.
As is fairly common 
(e.g., see~\cite{bannister2013force,battista1999graph,fruchterman1991graph,gajer2004multi,hu2005efficient,kamada1989algorithm,kobourov2013}),
let us define $F^{(a)}$ 
to be a spring-type force with idealized length $1$, so that,
for $p_u=(x_u,y_y)$ and $p_v=(x_v,y_v)$,
\[
F^{(a)}_{u,v}(p_u,p_v) ~=~ (d(p_u,p_v)^2-1)^2 
                       ~=~ ((x_u-x_v)^2 + (y_u-y_v)^2 -1)^2,
\]

\noindent
where, for the sake of simplicity, 
and as is common (see, e.g., \cite{gajer2004multi}),
we use squared distance to avoid a square-root, since 
$d(p_u,p_v)= d(p_u,p_v)^2$ when $d(p_u,p_v)= 1$.
As is also reasonably common 
(e.g., see~\cite{bannister2013force,fruchterman1991graph}),
let us define $F^{(r)}(p_u,p_v)$ to be a step function, which in this case is 
$1$ if $d(p_u,p_v)^2 < 1$ and is $0$ otherwise.
Finally, set $\mathbb{E}=0$, and let this be an instance of the
Optimal Force-Directed Graph Drawing problem.
By this construction, if there is a placement, $\Gamma$,
for $G$,
such that $\mathbb{E}_\Gamma\le \mathbb{E}$, then $\mathbb{E}_\Gamma=0$; hence, 
by the $F^{(a)}$ force in this construction,
every edge in the placement $\Gamma$ has length exactly $1$.
Moreover, by the $F^{(r)}$ force in this construction,
every pair of vertices, $u$ and $v$, with $u\not=v$, has
distance at least $1$.
Suppose, for the sake of contradiction, 
that the line segments representing 
two edges, $e$ and $f$, in this placement, $\Gamma$, cross.
In this case, 
the segments for
$e$ and $f$ form the diagonals of a quadrilateral, $Q$.
Moreover, because $Q$ is a quadrilateral,
at least one of the angles, $\alpha$, of $Q$ must be at least $90^\circ$;
hence, the diagonal (a segment corresponding to $e$ or $f$) 
opposite $\alpha$ is strictly longer than the two sides of $Q$
adjacent to $\alpha$. 
Thus, there are two vertices in the placement $\Gamma$
at distance less than $1$, which contradicts the fact that $\mathbb{E}_\Gamma=0$,
since all the values of $F^{(a)}$ and $F^{(r)}$ are non-negative.
Therefore, $\Gamma$ is a planar drawing of $G$.
Accordingly, there exists a unit-length planar drawing of $G$ if and only
if there is a solution to this instance of Optimal Force-Directed
Graph Drawing.
\end{proof}


